Analyzing the Impact of the Automatic Ball Strike System in Professional Baseball through a Case Study on KBO League Data

Recent advancements in professional baseball have led to the introduction of the Automated Ball-Strike (ABS) system, or ``robot umpires,'' which utilize machine learning, computer vision, and precise tracking technologies to automate ball-strike calls. The Korean Baseball Organization (KBO) league became the first professional baseball league to implement ABS during the 2024 season. Leveraging pitch data from 2,515 KBO games across multiple seasons and employing mathematical modeling, we examine the aggregate decision tendencies of human umpires versus those of the ABS within the ``gray zone'' of the strike zone. We propose and answer four research questions to examine the differences between human and robot umpires, player adaptation to ABS, assess the ABS system's fairness and consistency, and analyze its strategic implications for the game. Our findings offer valuable insights into the impact of technological integration in sports officiating, providing lessons relevant to future implementations in professional baseball and beyond.

==> sec/temp.tex <==

The introduction of the Automatic Ball-Strike System (ABS) marks a significant advancement in baseball games, promising precise ball-strike classification while minimizing human error.
Leveraging cutting-edge computer vision technology and data science in sports analytics, ABS offers highly accurate predictions, making its practical deployment a feasible reality.
The decision by the South Korea Baseball Organization (KBO) to adopt ABS starting in 2024 represents a milestone, marking the first usage of such technology in a professional baseball league.
This revolutionary shift is expected to profoundly impact both the game itself and its players.
Traditionally, ball-strike decisions in baseball have relied on human umpires, who may have inherent biases or preferences when judging whether a ball crosses the strike zone.
As a result, pitches with identical trajectories and placements can lead to different calls, even from the same umpire on the same day.
Moreover, variations in the strike zone, influenced by factors like the hitter's height, worsen the inconsistency and inaccuracy of these decisions.
Over time, umpires may develop tendencies to make consistently lenient or strict calls within specific zones, further impacting players' judgment and the overall fairness of the game.

Moreover, it's not uncommon for players to exploit the biased and inaccurate calls made by human umpires. For example, at the beginning of the games, pitchers frequently aim their throws near the boundary between balls and strikes to test the umpire's inclinations. If an umpire consistently favors a particular zone, pitchers may strategically target or avoid that area. Additionally, catchers employ techniques namely "framing" where they subtly manipulate the presentation of a pitch to make it appear as though it's within the strike zone, even if it's actually out of the zone. However, it's important to highlight that the introduction of ABS is expected to mitigate such tactics that have traditionally existed in baseball games. ABS brings a new level of objectivity and consistency to ball-strike calls, effectively reducing the influence of human biases and preferences. By automatically classifying balls and strikes with high precision, ABS aims to provide fair and accurate decisions in every game situation. This technological advancement not only enhances the integrity of the sport but also promotes a more level playing field for all teams and players. Additionally, ABS offers opportunities for further advancements in baseball analytics, providing valuable insights into player performance and game strategies.

Despite the advantageous aspects mentioned earlier, the ambitious introduction of ABS by the KBO may still require some refinements.
This transition to a new system necessitates adaptation from the players.
Previously reliant on human judgment and experience, the ball-strike calls are now automated, prompting players to adopt a new approach.
Moreover, there may be a need for additional fine-tuning for the fairness and reliability of the robot umpires.
The players' adaptation to these changes will take time, and the teams should provide training and support to effectively counter the ABS.
In this paper, our objective is to analyze pitching data from four different years to elucidate the fundamental disparities between human umpires and robot umpires, particularly focusing on the core-difference region namely the `gray zone'.
This analysis aims to provide valuable insights for players and teams to adapt to the introduction of robot umpires.
To address this goal, we pose three research questions:

\noindent{$\bullet$ \textbf{ RQ1:} Is there a significant difference between the calls made by human umpires and robot umpires?}

\noindent{$\bullet$ \textbf{ RQ2:} Where does the gray zone lie and what is the difference?}

\noindent{$\bullet$ \textbf{ RQ3:} Are the players adjusting to ABS?}

By addressing these research questions, our objective is to deepen the understanding of the gray zone phenomenon and its impact on the game of baseball.
Furthermore, we aim to elucidate the potential effects of ABS on baseball games with diverse perspectives under the consideration of factors in baseball games and provide insights into strategies for players and trainers to navigate this transition.
It is important to emphasize that the code and data utilized in this study will be made publicly accessible to ensure transparency and reproducibility, thereby fostering further research in this area.
To summarize, our work has three-folded contributions as follows.

\noindent{$\bullet$ \textbf{ SMTH:}}

\noindent{$\bullet$ \textbf{ SMTH:}}

\noindent{$\bullet$ \textbf{ SMTH:}}
